Measurement of the B^0 meson properties using partially reconstructed B^0 to D^{*-}pi^+ and B^0 to D^{*-}l^+nu decays with the BABAR detector

The two B^0 decay processes B^0 --> D^{*-}pi^+ and B^0 --> D^{*-}l^+nu have been studied by means of a partial reconstruction technique using a data sample collected with the BABAR detector at the PEP-II storage ring. To increase statistics, only the soft pi^- from the decay D^{*-} --> pi^-D^0 was used in association with either an oppositely-charged high-momentum pion or lepton. Events were then identified by exploiting the constraints from the simple kinematics of Y(4S) decays. A clear signature is obtained in each case. The position of the B^0 decay point was obtained from the reconstructed pi^+(l^+)pi^- vertex. The position of the other anti-B^0 in the event was also determined. Taking advantage of the boost given to the Y(4S) system by the asymmetric beam energies of PEP-II, the lifetime of the B^0 meson has been measured from the separation distance between the two vertices along the beam direction. The preliminary results are tau_B0 = 1.55+/-0.05+/-0.07 ps, tau_B0 = 1.62+/-0.02+/-0.09 ps, respectively for the B^0 --> D^{*-}pi^+ and B^0 --> D^{*-}l^+nu channels.

==> lds/lds_summary.tex <==
The \Bzb lifetime has been measured in a high statistics sample of \BtoDs\ decays.
The preliminary result is 
\ba
\nonumber \tBz = (1.63 \pm 0.01 \mathrm(stat.) \pm 0.09 \mathrm(syst.)) ~ps
\ea
were the study of the systematic error is still preliminary.\\
A preliminary study of the \BzBzb\ oscillation fenomenum has been presented, showing a clear evidence of
a time dependent asymmetry.

